Factor Graph Attention

Dialog is an effective way to exchange information, but subtle details and nuances are extremely important. While significant progress has paved a path to address visual dialog with algorithms, details and nuances remain a challenge. Attention mechanisms have demonstrated compelling results to extract details in visual question answering and also provide a convincing framework for visual dialog due to their interpretability and effectiveness. However, the many data utilities that accompany visual dialog challenge existing attention techniques. We address this issue and develop a general attention mechanism for visual dialog which operates on any number of data utilities. To this end, we design a factor graph based attention mechanism which combines any number of utility representations. We illustrate the applicability of the proposed approach on the challenging and recently introduced VisDial datasets, outperforming recent state-of-the-art methods by 1.1% for VisDial0.9 and by 2% for VisDial1.0 on MRR. Our ensemble model improved the MRR score on VisDial1.0 by more than 6%.

==> main.tex <==
% !TEX root =  egpaper_for_review.tex


\noindent
In this supplementary material we provide additional quantitative (see \secref{sec:quan}) and qualitative (see \secref{sec:qual}) results. 

\section{Quantitative Evaluation}
\label{sec:quan}

\noindent
\textbf{Ensemble model for VisDial v0.9:} For VisDial v1.0, a simple ensemble technique has significantly improved the results as discussed in the main paper. We observe a similar effect for VisDial v0.9, pushing the current state of the art for MRR from 0.6525 to 0.6892 as summarized in \tabref{tab:abl-atten}. 
We achieve this result with an ensemble of 9 models which differ only by the initial seed. For VisDial v1.0 we report a 5 model ensemble score. Due to restriction of the number of submissions to the evaluation server we could not evaluate a larger ensemble model.  The results in \tabref{tab:abl-atten} suggest that the VisDial v1.0 score in the paper can be further improve with a larger ensemble model. 

\noindent
\textbf{Analysis of Factor Graph Attention weights:} To infer the attention belief for a utility, \ie, $ b_i(u_i) $, we aggregate marginalized joint and local interactions and also local-information and prior terms. To calibrate each cue, we use scalar weights, \ie, $ \hat w_i, w_i, w_{i, j} $.  To obtain a better understanding of the reasoning process and analyze attention, we suggest an importance score:
\be
S(\gamma) = \frac{|m_\gamma\cdot \gamma|}{\sum_{\delta\in\{\hat w_i, w_i, (w_{i, j})_{j\in{\mathcal U}}\}} |m_\delta\cdot \delta|},
\label{eq:score}
\ee
where $ \gamma \in \{\hat w_i, w_i, (w_{i, j})_{j\in{\mathcal U}}\}$ is the weight  of a cue and $m_\gamma$ is the mean term of the corresponding cue $ \gamma $, which was calculated over the entire validation set. Note that $ \gamma $ are the scalar weights. 
%Also note that we use the shorthand $(\cdot)_i$
%\idan{I'm not sure how to notate this}
$ S(w_{i, j}) $ $\forall j\in {\mathcal U}$ captures the importance of the $ j $-th cue for utility $ i $. A high score means the $ i $-th utility attention belief heavily relies on  cue $ j $. Similarly, $ S(w_{i, i}), S(w_{i}) $, $ S(\hat w_{i}) $  capture the importance of local-interactions, local-information and prior cues for the $ i $-th utility. We report the scores in \tabref{tab:weights}. We observe that the answer utility relies mostly on local-interactions. The question heavily relies on the prior, but also makes use of history answers and question cues. The caption ignores all utilities other than the prior. The image question utility is the most important cue. Interestingly, we observe importance of priors. Image attention relies on the captions, while the caption  ignores all the cues and preserves the prior behavior. The history question and answers rely on the question and the local factors.  


\noindent
\textbf{Computation and insignificant interactions:}
%Despite the flexibility the factor graph brings in into the attention model, the proposed work considers some insignificant interactions between utilities (e.g., the caption is less important to the answer than the question or image) which leads to higher computation complexity. 
%
Upon training interactions may  be found to be unnecessary. %, and could be removed to speed up learning.
Our model can be optimized easily: 1)  The score in \equref{eq:score},  can be used to omit  less significant interactions. Previous multimodal attention doesn't model  pairwise interaction scores, making it hard to eliminate computations. 2) For the same image but different question, we can re-use calculated joint interactions, such as local-interaction, image-caption, \etc. This is impossible for approaches that pool  cues since the question changes. 3) As mentioned in Sec. 4.2, it's possible to share weights between similar utilities,  \eg, different history questions/answers. %\idan{4. It is always possible to remove interactions based on prior knowledge the flexibility of our model is superior versus previous approaches.} %, but this can be extended to a general image-text interactions depending on the problem etc. 

%
Currently, we don't consider  most of those options, as the model  trains quickly (8 hours vs.\ 33 hours of previous state-of-the-art) and fits into a single 12GB GPU. % with 12GB of memory.





\begin{figure}[t]
	\begin{center}
		\includegraphics[width=1\linewidth]{figs/potentials.pdf}
	\end{center}
	\vspace{-0.5cm}
	\caption{Two  images each with two  questions. We illustrate scores obtained from different types of factors.  Local-info denotes  `Image-Local-Information,' % obtained via local-information factor function,  
		Question refers to `Image-Question,' \etc. % obtained for each region by aggregating all image-question joint interactions messages with this region, \etc. 
		We observe `Image-Question' to have the highest variance between different questions, since its heat map differs the most. `Image-Question' also correlates the most with the final attention.}
	\label{fig:long}
	\label{fig:onecol}
	\vspace{-0.5cm}
\end{figure}


\begin{table}[b]
\centering
\begin{tabular}{cc}
\begin{minipage}[t]{0.5\linewidth}
	\centering
	\caption{Analysis of ensemble models for VisDial v0.9. With an ensemble of 9 models we observe an improvement of more than 3\% over the single model.}	
	\resizebox{\linewidth}{!}{%
		\begin{tabular}{lccccc}
			\Xhline{2\arrayrulewidth}
			\vspace{2pt}
			Model    & MRR    & R@1  & R@5   & R@10  & Mean  \\ \hline
			FGA   & 0.6525 & 51.43 & 82.08 & 89.56 & 4.35 \\
			Ensemble of 2 FGA & 0.6711 & 53.56 & 83.83 & 90.97 & 3.92 \\
			Ensemble of 3 FGA & 0.6786 & 54.28 & 84.71 & 91.69 & 3.73 \\ 
			Ensemble of 4 FGA & 0.6819 & 54.56 & 85.19 & 92.10 & 3.62 \\
	        Ensemble of 5 FGA & 0.6848 & 54.82 & 85.57 & 92.38 & 3.55 \\ 
	        Ensemble of 6 FGA & 0.6860 & 54.95 & 85.71 & 92.52 & 3.50 \\
	        Ensemble of 7 FGA & 0.6869 & 54.97 & 85.91 & 92.67 & 3.47 \\
	        Ensemble of 8 FGA & 0.6881 & 55.10 & 86.04 & 92.77 & 3.44 \\
	        Ensemble of 9 FGA & \textbf{0.6892} & \textbf{55.16} & \textbf{86.26} & \textbf{92.95} & \textbf{3.39} \\ 		
			\Xhline{2\arrayrulewidth}
		\end{tabular}}
		
		\label{tab:abl-atten}
\end{minipage}
&
\begin{minipage}[t]{0.5\linewidth}
\centering
		\caption{For each utility (column) we show the three most related cues based on the $ S $ score given in \equref{eq:score}. We provide $ S $ in parenthesis. $P$, $L_1$ and $L_2$ indicate prior, local-information and local-interactions of the utility in the  column.}
		\resizebox{\linewidth}{!}{%
		\begin{tabular}{@{}l|l|l|l|l|l@{}}
			\Xhline{2\arrayrulewidth}
			\vspace{2pt}
			A               & Q               & C           & I         & $ H_Q $   & $ H_A $ \\ \hline
			$ L_1 $ (0.125)   & $ P (0.851 ) $  & $ P $ ( 0.988 ) & $ Q $ (0.593) & $ Q $ (0.205) & $ L_2 $  (0.607) \\
			$ H_Q $ (0.122) & $ H_A (0.052) $ & $ I $ ( 0.004)  & $ L_1 $ (0.186) & $ L_1 $ (0.121) & $ Q $ (0.304) \\
			$ Q $ (0.075)       & $ H_Q (0.031) $ & $ A $ (0.001)   & $ C $ (0.123) & $ L_2 $ (0.085) & $ L_1 $ (0.017) \\
			\Xhline{2\arrayrulewidth}
		\end{tabular}}
		\label{tab:weights}
\end{minipage}
\end{tabular}
\end{table}

%\begin{table}[t]
%		\centering
%		\caption{For each utility (column) we show the three most related cues and provide their weight in parenthesis. $P$, $L_1$ and $L_2$ indicate prior, local-information and local-interactions of the utility in the  column.}
%		\resizebox{\linewidth}{!}{%
%		\begin{tabular}{@{}l|l|l|l|l|l@{}}
%			\Xhline{2\arrayrulewidth}
%			\vspace{2pt}
%			A               & Q               & C           & I         & $ H_Q $   & $ H_A $ \\ \hline
%			$ L_1 $ (0.125)   & $ P (0.851 ) $  & $ P $ ( 0.988 ) & $ Q $ (0.593) & $ Q $ (0.205) & $ L_2 $  (0.607) \\
%			$ H_Q $ (0.122) & $ H_A (0.052) $ & $ I $ ( 0.004)  & $ L_1 $ (0.186) & $ L_1 $ (0.121) & $ Q $ (0.304) \\
%			$ Q $ (0.075)       & $ H_Q (0.031) $ & $ A $ (0.001)   & $ C $ (0.123) & $ L_2 $ (0.085) & $ L_1 $ (0.017) \\
%			\Xhline{2\arrayrulewidth}
%		\end{tabular}}
%		\label{tab:weights}
%\end{table}
%
%\begin{table}[t]
%	\centering
%	\caption{Analysis of ensemble models for VisDial0.9. With ensemble of 8 models we observe an improvement of 3\% over the single model.}	
%	\resizebox{\linewidth}{!}{%
%		\begin{tabular}{lccccc}
%			\Xhline{2\arrayrulewidth}
%			\vspace{2pt}
%			Model    & MRR    & R@1  & R@5   & R@10  & Mean  \\ \hline
%			FGA   & 0.6525 & 51.43 & 82.08 & 89.56 & 4.35 \\
%			Ensemble of 2 FGA & 0.6711 & 53.56 & 83.83 & 90.97 & 3.92 \\
%			Ensemble of 3 FGA & 0.6786 & 54.28 & 84.71 & 91.69 & 3.73 \\ 
%			Ensemble of 4 FGA & 0.6819 & 54.56 & 85.19 & 92.10 & 3.62 \\
%	        Ensemble of 5 FGA & 0.6848 & 54.82 & 85.57 & 92.38 & 3.55 \\ 
%	        Ensemble of 6 FGA & 0.6860 & 54.95 & 85.71 & 92.52 & 3.50 \\
%	        Ensemble of 7 FGA & 0.6869 & 54.97 & 85.91 & 92.67 & 3.47 \\
%	        Ensemble of 8 FGA & \textbf{0.6881} & \textbf{55.10} & \textbf{86.04} & \textbf{92.77} & \textbf{3.44} \\ 		
%			\Xhline{2\arrayrulewidth}
%		\end{tabular}}
%		
%		\label{tab:abl-atten}
%	\end{table}
	
	
\clearpage

\section{Qualitative Evaluation}
\label{sec:qual}

\noindent
\textbf{Factors visualization:} 
We  provide additional visualization in \figref{fig:onecol}. We visualize scores for each image region obtained from different types of factors. %In fig.1 we see several interactions. 
`Image-Local-Information,' `Image-Caption' and `Image-Local-Interaction' are constant for different questions, while  `Image-Question,' `Image-Answer,' `Image-History-Q' and `Image-History-A' change for every question. We calculated the variance of interactions and observe that `Image-Question'  has the highest variance ($\approx 3$), while `Image-Answer,' `Image-History-Q' and `Image-History-A' have a variance of $\approx 1$.  Beyond the importance score, the high-variance also suggests that the `Image-Question' cue is most important. %, as also seen in our importance score. 

\noindent
\textbf{Attention over  dialogs:} In \figref{fig:res}, we present a randomly-picked set of 50 images along with their corresponding dialogs. An automatic script is used to generate the figures.  We highlight that image attention is aware of the scene in the question context, and able to attend to correct foreground or background regions.  Question attention attends to informative words, and answer attention frequently correlates with the predicted answer.  History attention emphasizes nuances. 

\clearpage

\begin{figure*}[t]
	\caption{50 dialogs along with question, answers and history attention. The predicted answer (\ie, A) and ground-truth answer (\ie, GT) are also provided.  %Note: Caption attention is not shown here, as the attention always focus on the last word due to priors.
	}
		\label{fig:res}
			\subfloat{\includegraphics[width=0.87\linewidth]{figs/supp/final73}}
\end{figure*}
\begin{figure*}[t]
	\ContinuedFloat
	\centering
	\subfloat{\includegraphics[width=0.87\linewidth]{figs/supp/final71}}
\end{figure*}
\begin{figure*}[t]
	\ContinuedFloat
	\centering
	\subfloat{\includegraphics[width=0.87\linewidth]{figs/supp/final87}}
\end{figure*}
\begin{figure*}[t]
	\ContinuedFloat
	\subfloat{\includegraphics[width=0.87\linewidth]{figs/supp/final72}}
\end{figure*}
\begin{figure*}[t]
	\ContinuedFloat
	\subfloat{\includegraphics[width=0.87\linewidth]{figs/supp/final160}}
\end{figure*}
\begin{figure*}[t]
	\ContinuedFloat
	\subfloat{\includegraphics[width=0.87\linewidth]{figs/supp/final150}}
\end{figure*}
\begin{figure*}[t]
	\ContinuedFloat
	\subfloat{\includegraphics[width=0.87\linewidth]{figs/supp/final162}}
\end{figure*}
\begin{figure*}[t]
	\ContinuedFloat
	\subfloat{\includegraphics[width=0.87\linewidth]{figs/supp/final148}}
\end{figure*}
\begin{figure*}[t]
	\ContinuedFloat
	 \subfloat{\includegraphics[width=0.87\linewidth]{figs/supp/final6}}
\end{figure*}
\begin{figure*}[t]
	\ContinuedFloat
	\subfloat{\includegraphics[width=0.87\linewidth]{figs/supp/final124}}
\end{figure*}
\begin{figure*}[t]
	\ContinuedFloat
	\subfloat{\includegraphics[width=0.87\linewidth]{figs/supp/final125}}
\end{figure*}
\begin{figure*}[t]
	\ContinuedFloat
	\subfloat{\includegraphics[width=0.87\linewidth]{figs/supp/final151}}
\end{figure*}
\begin{figure*}[t]
	\ContinuedFloat
	\subfloat{\includegraphics[width=0.87\linewidth]{figs/supp/final153}}
\end{figure*}

\clearpage


